Disturbance Observers for Robust Safety-critical Control with Control Barrier Functions

This work provides formal safety guarantees for control systems with disturbance. A disturbance observer-based robust safety-critical controller is proposed, that estimates the effect of the disturbance on safety and utilizes this estimate with control barrier functions to attain provably safe dynamic behavior. The observer error bound - which consists of transient and steady-state parts - is quantified, and the system is endowed with robustness against this error via the proposed controller. An adaptive cruise control problem is used as illustrative example through simulations including real disturbance data.

==> Disturbance Observer ISSf CBF/_Aux/preamble.tex <==
% Text Appearance
% ----------------------
%\usepackage{palatino}
%\usepackage{mathpazo}
\usepackage{times}
% \usepackage[parfill]{parskip}
\usepackage{setspace}
\usepackage{url}
\spacing{1}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
% Graphics
% ------------
\usepackage{graphicx}		% For \includegraphics
%\graphicspath{{figures/}}	% Looks under figures/ sub-dir for files referenced by \includegraphics
%\usepackage{subcaption}
\usepackage{wrapfig}
%\usepackage[format=plain,font=footnotesize,labelfont=bf,labelsep=period]{caption}
\usepackage{sidecap} % For sidecaptions for figures
%\usepackage{subfig}
\usepackage[export]{adjustbox}
% \usepackage{subcaption}
%\usepackage[font=small]{caption}
\usepackage{float}
% \usepackage{subfigure}
% \usepackage{color, soul}
\let\proof\relax \let\endproof\relax 

\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{amsthm}
\usepackage{mathtools}
% \usepackage{pdfsync}
\usepackage[normalem]{ulem}
\usepackage{paralist}	% For enumerations with better titled numbers
\usepackage[space]{grffile} % Space in filenames
\usepackage{color}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{bm}
\usepackage{cancel}
\usepackage{hhline}


\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
\theoremstyle{definition}
\newtheorem{assumption}{Assumption}
\theoremstyle{definition}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}

\newcommand{\N}{\mathbb{N}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\until}[1]{[#1]}
\newcommand{\map}[3]{#1:#2 \rightarrow #3}
\newcommand{\Sc}{\mathcal{S}}

\newcommand{\longthmtitle}[1]{{\rm \textbf{(#1).}}}
\newcommand{\setdef}[2]{\{#1 \; : \; #2\}}
\newcommand{\setdefb}[2]{\big\{#1 \; : \; #2\big\}}
\newcommand{\setdefB}[2]{\Big\{#1 \; : \; #2\Big\}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\K}{\mathcal{K}}

\newcommand{\xdot}{\dot{x}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Xcal}{\mathcal{X}}

\newcommand{\Rplus}{\R_{\geq 0}}

\newcommand{\classK}{\mathcal{K}}
\newcommand{\classKinfty}{\mathcal{K}_{\infty}}
\newcommand{\classKL}{\mathcal{KL}}

\newcommand{\q}{q}
\newcommand{\dq}{\dot{q}}
\newcommand{\ddq}{\ddot{q}}

\newcommand{\gap}{\vspace{.1cm}}
\newcommand{\gaps}{\vspace{.1cm}}

\newcommand{\newsec}[1]{\gap {\bf \noindent #1 }}
\newcommand{\thetadot}{\dot{\theta}}
\newcommand{\qdot}{\dot{q}}

\newcommand{\Kinfinity}{\classKinfty}
\newcommand{\KLinfinity}{\classKL}
\newcommand{\etavar}{\eta}


\newcommand{\Kclf}{K_{\mathrm{clf}}}
\newcommand{\Kcbf}{K_{\mathrm{cbf}}}
\newcommand{\Kcsf}{K_{\mathrm{csf}}}
\newcommand{\Krcbf}{K_{\mathrm{cbf}}}
\newcommand{\Kzcbf}{K_{\mathrm{csf}}}


\definecolor{blue}{RGB}{38,38,134}
\definecolor{darkblue}{RGB}{0,0,102}
\definecolor{lightblue}{RGB}{77,77,148}

\definecolor{gold}{RGB}{234, 170, 0}
\definecolor{metallic_gold}{RGB}{139, 111, 78}

\newcommand{\fmtStability}[1]{{\color{blue} #1}}
\newcommand{\fmtSafety}[1]{{\color{red} #1}}
\newcommand{\fmtEfficiency}[1]{{\color{darkgreen} #1}}
\newcommand{\fmtForce}[1]{{\color{maroon} #1}}

\newcommand{\ext}{{\mathrm{ext}}}
\newcommand{\dev}{{\mathrm{robot}}}
\newcommand{\des}{{\mathrm{des}}}
\newcommand{\Aforce}{A_{F}}
\newcommand{\bforce}{b_F}
\newcommand{\unifiedcontroller}{\fmtEfficiency{Unified Controller} }
\newcommand{\defeq}{\triangleq}

\renewcommand{\cal}[1]{\mathcal{ #1 }}
\newcommand{\mb}[1]{\mathbf{ #1 }}
\newcommand{\bs}[1]{\boldsymbol{ #1 }}
\newcommand{\bb}[1]{\mathbb{ #1 }}
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert}
\newcommand{\der}[2]{\frac{\mathrm{d} #1 }{\mathrm{d} #2 }}
\newcommand{\derp}[2]{\frac{\partial #1 }{\partial #2 }}

\newcommand{\interior}{\mathrm{int}}
\newcommand{\grad}{\nabla}
\newcommand{\intersect}{\cap}
\newcommand{\union}{\cup}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator{\sgn}{sgn}

%\newcommand{\new}[1]{{\color{red} #1}}

\usepackage{xfrac}
\newcommand*\rfrac[2]{{}^{#1}\!/_{#2}}
\usepackage{dblfloatfix}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

\usepackage{cite}
\usepackage[dvipsnames,table,xcdraw]{xcolor}



\usepackage{amsfonts}
\usepackage{algorithmic}
\usepackage{textcomp}

\usepackage{subfigure}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{widetext}
%\usepackage{_Aux/lcsys}
